P4DB -- The Case for In-Network OLTP (Extended Technical Report)

In this paper we present a new approach for distributed DBMSs called P4DB, that uses a programmable switch to accelerate OLTP workloads. The main idea of P4DB is that it implements a transaction processing engine on top of a P4-programmable switch. The switch can thus act as an accelerator in the network, especially when it is used to store and process hot (contended) tuples on the switch. In our experiments, we show that P4DB hence provides significant benefits compared to traditional DBMS architectures and can achieve a speedup of up to 8x.

==> 07_Deployments.tex <==
\section{Other Deployments}
\label{sec:deployments}


While \system{} focuses only on a single-tenant DBMS deployment in a rack with a top-of-the rack switch, other deployments are also conceivable, which we briefly sketch in the following.

\vspace{-1.5ex}\paragraph{Switch Hierarchies.}
Data center networks that provide connectivity between nodes often build on hierarchies with multiple switches: The lowest layer consisting of top-of-the-rack (ToR) switches bundles a subset of nodes together to ensure low-latency communication and high throughput, while multiple ToR switches are then cross-connected in subsequent layers to provide connectivity to all nodes.
Using such switch hierarchies, \system{} can make use of the information about the topology to improve performance. For example, the nearest programmable switch running \system{} could be used for offloading to avoid sending packets through a long path consisting of multiple hops.
Another use-case could be to utilize multiple switches for replication, to ensure that the system is robust against failures by leveraging protocols such as \cite{jin2018netchain}.


\vspace{-1.5ex}\paragraph{Multi-Tenancy}
Multi-tenancy means in our context that a single instance of \system{}  serves multiple customers. Such a multi-tenancy setup for different customers is actually covered already by benchmarks such as SmallBank or TPC-C that we include in our evaluation in Section \ref{sec:evaluation}.
While tenants typically share the same database schema in such a setup, in addition, data of each tenant needs to be isolated to remain invisible to other tenants. This is generally possible in \system{} by partitioning the switch resources, thus making it impossible to access or modify data from other tenants.
However, the limited switch resources then still need to be kept in mind when deciding which hot tuples are offloaded to the switch.



